A Review on Deep-Learning Algorithms for Fetal Ultrasound-Image Analysis

Deep-learning (DL) algorithms are becoming the standard for processing ultrasound (US) fetal images. Despite a large number of survey papers already present in this field, most of them are focusing on a broader area of medical-image analysis or not covering all fetal US DL applications. This paper surveys the most recent work in the field, with a total of 145 research papers published after 2017. Each paper is analyzed and commented on from both the methodology and application perspective. We categorized the papers in (i) fetal standard-plane detection, (ii) anatomical-structure analysis, and (iii) biometry parameter estimation. For each category, main limitations and open issues are presented. Summary tables are included to facilitate the comparison among the different approaches. Publicly-available datasets and performance metrics commonly used to assess algorithm performance are summarized, too. This paper ends with a critical summary of the current state of the art on DL algorithms for fetal US image analysis and a discussion on current challenges that have to be tackled by researchers working in the field to translate the research methodology into the actual clinical practice.

==> overall_summary.tex <==

\begin{table*}[tbp]
    \centering
        \caption{\label{table:papers_analysed}
         Summary of all articles found, sorted according to review organization}
    \begin{adjustbox}{width=.98\textheight, angle=0}
    \begin{tabular}{cccccc}
    \hline
    Article & Organ & Dataset & Method 
    \\
    \hline
    \rowcolor{languidlavender}
    Wu et al. (2017) \cite{wu2017fuiqa} & \pbox{30cm}{Abdomen} & \vtop{\hbox{\strut 8072 2D-US (492 US videos) (train)}\hbox{\strut + 2606 2D-US (219 US videos) (test)}}& Localization + classification CNN &
    \vtop{\hbox{\strut AUC = 0.99, Acc = 0.98}\hbox{\strut Sen = 0.96, Spec = 0.97}}
    \\
    Chen et al. (2017) \cite{chen2017ultrasound} & \pbox{30cm}{Abdomen, face and thorax} & \vtop{\hbox{\strut 37376 2D-US (900 US videos) (train)}\hbox{\strut + 13248 2D-US (331 US videos) (test)}} & Multitask localization/classification CNN & \vtop{\hbox{\strut Acc = 0.87, Prec = 0.71}\hbox{\strut Rec = 0.64, F1 = 0.64}} 
    \\
    \rowcolor{languidlavender}
    Yu et al. \cite{yu2017deep} (2017) & Face & \vtop{\hbox{\strut 4849 2D-US (train)}\hbox{\strut + 2418 2D-US (test)}}& Classification CNN & \vtop{\hbox{\strut AUC = 0.99, Acc = 0.96}\hbox{\strut Prec = 0.96, Rec = 0.97}\hbox{\strut F1 = 0.97}} 
    \\
    Qu et al, \cite{qu2020standard} (2020) & Brain & \vtop{\hbox{\strut 30.000 2D-US images which}\hbox{\strut are split in 5 folds}}& Classification CNN & \vtop{\hbox{\strut Acc = 0.93, Prec = 0.93}\hbox{\strut Rec = 0.92, F1 = 0.93}}
    \\
    \rowcolor{languidlavender}
    Burgos-Artizzu et al \cite{burgos2020evaluation} (2020) & \vtop{\hbox{\strut Abdomen, brain, femur,}\hbox{\strut thorax, maternal cervix}} & \vtop{\hbox{\strut 7129 2D-US (896 patients) (train)}\hbox{\strut 5271 2D-US (896 patients) (test)}} & Classification CNN & \vtop{\hbox{\strut 6.2 \% top-1 error,}\hbox{\strut 0.27 \% top-3 error}\hbox{\strut Acc = 0.94}}
    \\
    Sridar et al \cite{sridar2019decision} (2019) & \vtop{\hbox{\strut Abdomen, arm, blood vessels}\hbox{\strut cord insertion, face, femur}\hbox{\strut foot, genitals, brain, thorax}\hbox{\strut kidney, leg, spine, hand}} & \vtop{\hbox{\strut 3109 2D-US (train)}\hbox{\strut + 965 2D-US (test)}}  & CNN feature extraction + SVM & \vtop{\hbox{\strut Acc = 0.97, Prec = 0.76}\hbox{\strut Rec = 0.75}}
    \\
    \rowcolor{languidlavender}
    Pu et al. \cite{pu2021automatic} (2021) & Abdomen, brain, spine & \vtop{\hbox{\strut 67.000 2D-US (1199 US videos) (train)}\hbox{\strut 16.740 2D-US (244 US videos) (test)}} & Classification CNN + RNN & \vtop{\hbox{\strut Acc = 0.85, Prec = 0.85}\hbox{\strut Rec = 0.85, F1 = 0.85}}
    \\
    Schlemper et al. \cite{schlemper2019attention} (2018) & \vtop{\hbox{\strut Abdomen, brain, profile,}\hbox{\strut lips, kidney, femur}\hbox{\strut spine, thorax}} & - & Classification CNN + attention gate & \vtop{\hbox{\strut Acc = 0.98, Prec = 0.98}\hbox{\strut Rec = 0.93, F1 = 0.96}}
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> prova.tex <==

\clearpage
\onecolumn
\appendix

\begin{longtable}{\textwidth}{XXXXXX}
\textbf{A}&\textbf{B}\\
\caption{a long table\label{zzz}}
\endfirsthead
\textbf{A}&\textbf{B}\\
\caption*{a long table (continued)}
\endhead
Wu et al.,  \cite{wu2017fuiqa} (2017) & FASP & 8072 2D (492 videos) & 2606 2D (219 videos/66 women) & 3 & AUC=0.99, $Acc$=0.98, $Rec$=0.96, $Spec$=0.97\\
    
    Yu et al., \cite{yu2017deep} (2017) & FFSP & 4849 2D & 2418 FFSP 2D & Few & AUC=0.99, $Acc$=0.96, $Prec$=0.96, $Rec$=0.97, $F1$=0.97\\
    
    
    Qu et al., \cite{qu2020standard} (2020) & FBSPs & 4 out of 5 folds cross validation on 19142 2D (155 woman) &  1 out of 5 folds cross validation on 19142 2D (155 woman) & Few & $Acc$=0.93, $Prec$=0.93, $Rec$=0.92, $F1$=0.93\\
    
    Burgos-Artizzu et al., \cite{burgos2020evaluation} (2020) & Multiple & 7129 2D (896 women) & 5271 2D (896 women) & 1 &  6.2 \% top-1 error, 0.27 \% top-3 error, $Acc$ = 0.94 \\
    
    Sridar et al., \cite{sridar2019decision} (2019) & Multiple & 3109 2D & 965 2D & 1 & $Acc$ = 0.97, $Prec$ = 0.76, $Rec$ = 0.75\\
     
    Pu et al., \cite{pu2021automatic} (2021) & FASP, FTSP, FCSP, FLVSP & 68296 2D (1199 videos)&  16740 2D (244 videos) & Few & $Acc$ = 0.85, $Prec$ = 0.85, $Rec$ = 0.85, $F1$ = 0.85\\
    
    Chen et al., \cite{chen2017ultrasound} (2017) & FASP, FFASP, FFVSP & 37376 2D (900 videos/women) &  13248 2D (331 videos/women) & 1 & $Acc$=0.87, $Prec$=0.71, $Rec$=0.64, $F1$=0.64\\
    
    Kong et al. \cite{kong2018automatic} (2018) &
    4CH, FASP, FBSP, FFSPs & 17036 2D & 5678 2D  & 1 expert & $Prec$ = 0.98, $Rec$ = 0.98, $F1$ = 0.98  \\
    
    Liang et al., \cite{liang2019sprnet} (2019) & FASP, FBSP, FFSPs & 17840 2D & 4455 2D & & $Acc$ = 0.99, $Sen$ = 0.96, $Spec$ = 0.99, $F1$ = 0.95& \\
    
    Schlemper et al., \cite{schlemper2019attention} (2019) & Multiple & 122233 2D & 38243 2D  & Many & $Acc$ = 0.98, $Rec$ = 0.93, $Prec$ = 0.93, $F1$ = 0.93 \\
     
    Cai et al., \cite{cai2018multi} (2018) & FASP & 20 videos & 324 2D (5 videos/1 woman) & Few & $Prec$ = 0.96, $Rec$ = 0.96, $F1$ = 0.96 \\
    
    Sundaresan et al., \cite{sundaresan2017automated} (2017) & 4CH, LVOT, 3VV & 10000 2D (10 women) & 2178 2D (2 women) & 1&  error rate = 0.23 \\
    
    Cai et al., \cite{cai2020spatio} (2020) & FASP, FTVSP, FFESP & \textcolor{orange}{non se capisce} & \textcolor{orange}{non se capisce} & Few & $Prec$ = 0.98,  $Rec$ = 0.85, $F1$ = 0.87 \\
    
    %Patra et al. \cite{patra2021multimodal} & 2021 & & & &  \\
    
     
    Dong et al., \cite{dong2019generic} (2019) & 4CH & 4 out of 5 folds cross validation on 7032 2D images & 1 out of 5 folds cross validation on 7032 2D images & Few &  $mAP$ = 0.81\\
     
    Lee et al., \cite{lee2021principled} (2021) & Multiple & 2 out of 3 folds cross validation on 2256 2D & 1 out of 3 folds cross validation on 2256 2D & - & $Prec$ = 0.75, $Rec$ = 0.73, $F1$ = 0.74\\
    
    Lin et al., \cite{lin2018quality} (2018) & FBSP &&&& \\
    
    Lin et al., \cite{lin2019multi} (2019) & FBSP & 1451 2D & 320 2D & Few & $mAP$= 0.93\\
     
    Zhang et al., \cite{zhang2021automatic} (2021) & FASP, FBSP, 4CH & 2460 2D & 820 2D & 2 & $mAP$ = 0.94\\
     
    Baumgartner et al., \cite{baumgartner2017sononet} (2017) & Multiple & \textcolor{orange}{non se capisce}& 109165 2D (104722 only background) & 45 &  $Prec$ = 0.77, $Rec$ = 0.90 $F1$ = 0.80 and $IoU$ = 0.62 \\ 

    Li et al., \cite{li2018standard} (2018) & FVSP, FCSP & 50 3D (50 women) & 22 3D (22 women) & &mean plane centre difference = 3.44 mm, rotation angle = 11.05\degree\\ 
    
    Tsai et al., \cite{tsai2021automatic} (2021) &&&&& \\
    
    Dou et al., \cite{dou2019agent} (2019) &&&&& \\
    
    Yang et al., \cite{yang2021agent} (2021) &&&&& \\
    
    Yaqub et al., \cite{yaqub2017deep} (2017) &&&&& \\
    
    Gao et al., \cite{gao2020label} (2020) &&&&& \\
    
    Chen et al., \cite{chen2019self} (2019) &&&&& \\
    
    Tan et al., \cite{tan2019semi} (2019) &&&&& \\
    
    Meng et al., \cite{meng2020unsupervised} (2020) &&&&& \\
\end{longtable}
